Equidimensional Isometric Extensions

Let $\Sigma$ be a hypersurface in an $n$-dimensional Riemannian manifold $M$, $n\geqslant 2$. We study the isometric extension problem for isometric immersions $f:\Sigma\to\mathbb R^n$, where $\mathbb R^n$ is equipped with the Euclidean standard metric. We prove a general curvature obstruction to the existence of merely differentiable extensions and an obstruction to the existence of Lipschitz extensions of $f$ using a length comparison argument. Using a weak form of convex integration, we then construct one-sided isometric Lipschitz extensions of which we compute the Hausdorff dimension of the singular set and obtain an accompanying density result. As an application we obtain the existence of infinitely many Lipschitz isometries collapsing the standard two-sphere to the closed standard unit $2$-disk mapping a great-circle to the boundary of the disk.

==> convexintegration.tex <==
\psfrag{r}{$S^1_{r_2}(-1)$}
\psfrag{s}{$S^2_{r_1}(0)$}
\psfrag{t}{$S^0_{r_1}(0)$}
\psfrag{u}{$S^0_{r_2}(-1)$}

==> cutofflipschitz.tex <==
\psfrag{j}{$\ell$}
\psfrag{O}{$\overline{\Omega_\ell^c}$}
\psfrag{P}{$\bar\Omega_\ell$}
